Structural underpinnings of control in multiplex networks

To design control strategies that predictably manipulate a system's behavior, it is first necessary to understand how the system's structure relates to its response. Many complex systems can be represented as multilayer networks whose response and control can be studied in the framework of network control theory. It remains unknown how a system's layered architecture dictates its control properties, particularly when control signals can only access the system through a single input layer. Here, we use the framework of linear control theory to probe the control properties of a duplex network with directed interlayer links. We determine the manner in which the structural properties of layers and relative interlayer arrangement together dictate the system's response. For this purpose, we calculate the exact expression of optimal control energy in terms of layer spectra and the relative alignment between the eigenmodes of the input layer and the deeper target layer. For a range of numerically constructed duplex networks, we then calculate the control properties of the two layers as a function of target-layer densities and layer topology. The alignment of layer eigenmodes emerges as an important parameter that sets the cost and routing of the optimal energy for control. We understand these results in a simplified limit of a single-mode approximation, and we build metrics to characterize the routing of optimal control energy through the eigenmodes of each layer. Our analytical and numerical results together provide insights into the relationships between structure and control in duplex networks. More generally, they serve as a platform for future work designing optimal \emph{interlayer} control strategies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
